DragAPart: Learning a Part-Level Motion Prior for Articulated Objects

We introduce DragAPart, a method that, given an image and a set of drags as input, generates a new image of the same object that responds to the action of the drags. Differently from prior works that focused on repositioning objects, DragAPart predicts part-level interactions, such as opening and closing a drawer. We study this problem as a proxy for learning a generalist motion model, not restricted to a specific kinematic structure or object category. We start from a pre-trained image generator and fine-tune it on a new synthetic dataset, Drag-a-Move, which we introduce. Combined with a new encoding for the drags and dataset randomization, the model generalizes well to real images and different categories. Compared to prior motion-controlled generators, we demonstrate much better part-level motion understanding.

==> figures/rebuttal/addition-results.tex <==
\begin{figure}[ht!]
\includegraphics[trim={2px 0px 0px 0px}, clip, width=\linewidth]{figures/rebuttal/results.pdf}
\vspace{-1.5em}
\caption{
\textbf{More Results} on images captured \emph{in the wild}.
}%
\label{fig:rebuttal-results}
\end{figure}

==> figures/supmat/supmat-fig-additional-results-bg.tex <==
\begin{figure}[tb!]
\includegraphics[trim={0px 0px 0px -2px}, clip, width=\linewidth]{figures/supmat/additional-res-bg.pdf}
\begin{picture}(0,0)
    \put(18,522){\scriptsize Input}
    \put(65,522){\scriptsize Generation}
    \put(137,522){\scriptsize Input}
    \put(183,522){\scriptsize Generation}
    \put(254,522){\scriptsize Input}
    \put(302,522){\scriptsize Generation}
\end{picture}
\vspace{-1.5em}
\caption{
\textbf{Additional Qualitative Results}
on images with diverse backgrounds.
}%
\label{fig:additional-results-bg}
\end{figure}

==> tables/rebuttal/application-comp.tex <==
\begin{table}[ht!]
\small
\setlength\tabcolsep{5pt}
\setlength{\abovecaptionskip}{2pt} % Adjust the space above the caption
\renewcommand{\arraystretch}{1.0}
\centering
\begin{tabular}{@{}l cc@{}}
\toprule
& DragNUWA & DragAPart (ours) \\
\midrule
Mask IoU (\%) & 12.77 & \textbf{27.29} \\
\bottomrule
\end{tabular}
\caption{
\textbf{Comparison of Moving Part Segmentation} using features obtained with different drag-conditioned diffusion models.}
\label{tab:rebuttal-application}
\vspace{-0.25in}
\end{table}

==> tables/rebuttal/architecture-comp.tex <==
\begin{table}[ht!]
\small
\setlength\tabcolsep{5pt}
\setlength{\abovecaptionskip}{2pt} % Adjust the space above the caption
\renewcommand{\arraystretch}{1.0}
\centering
\begin{tabular}{@{}l ccc@{}}
\toprule
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
MLP & 21.24 & \textbf{0.925} & 0.067 \\
ConvNet & \textbf{21.38} & \textbf{0.925} & \textbf{0.066} \\
\bottomrule
\end{tabular}
\caption{
\textbf{Comparison of Flow Embedding Architectures.}}
\label{tab:rebuttal-architecture}
% \vspace{-0.25in}
\end{table}

% SD U-Net w/o RT & 21.38 & 0.925 & \textbf{0.066} & 18.03 & 0.897 & 0.104 \\
% SD U-Net & \textbf{21.82} & \textbf{0.928} & \textbf{0.066} & \textbf{19.74} & \textbf{0.920} & \textbf{0.083} \\

% \begin{table}[t]
% \small
% \setlength\tabcolsep{5pt}
% \renewcommand{\arraystretch}{1.0}
% \centering
% \begin{tabular}{@{}l ccc c ccc@{}}
% \toprule
% \multicolumn{3}{c}{\textbf{MLP}} && \multicolumn{3}{c}{\textbf{Convolutional}} \\
% \cline{1-3}
% \cline{5-7}
% PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ && PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
% \midrule
% 21.24 & \textbf{0.925} & 0.067 && \textbf{21.38} & \textbf{0.925} & \textbf{0.066} \\
% \bottomrule
% \end{tabular}
% \caption{
% \textbf{Comparison of Flow Embedding Architectures.}}
% \label{tab:rebuttal-architecture}
% \vspace{-0.2in}
% \end{table}
